Byzantine Stable Matching

In stable matching, one must find a matching between two sets of agents, commonly men and women, or job applicants and job positions. Each agent has a preference ordering over who they want to be matched with. Moreover a matching is said to be stable if no pair of agents prefer each other over their current matching. We consider solving stable matching in a distributed synchronous setting, where each agent is its own process. Moreover, we assume up to $t_L$ agents on one side and $t_R$ on the other side can be byzantine. After properly defining the stable matching problem in this setting, we study its solvability. When there are as many agents on each side with fully-ordered preference lists, we give necessary and sufficient conditions for stable matching to be solvable in the synchronous setting. These conditions depend on the communication model used, i.e., if parties on the same side are allowed to communicate directly, and on the presence of a cryptographic setup, i.e., digital signatures.

==> sty/macros.tex <==

%----- Algorithm Environment ----------------------------------
\RequirePackage{algpseudocode}
%Header for Algorithms/Functionalities
\newcommand{\algoHead}[1]{\vspace{0.2em} \underline{\textbf{#1}} \vspace{0.3em}}
\newcommand{\algoHeadExt}[2]{\vspace{0.2em} \underline{\textbf{#1} #2} \vspace{0.3em}}
%Multiline Algo-States
\makeatletter
\algnewcommand{\ExtendedState}[1]{\State
\parbox[t]{\dimexpr\linewidth-\ALG@thistlm}{\hangindent=\algorithmicindent\strut\hangafter=3#1\strut}}
\makeatother
%Algorithms States
\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
%Algo Comments
\algrenewcommand{\algorithmiccomment}[1]{{\color{gray}// #1}}
%Inline ifs
\algnewcommand{\IIf}[1]{\State\algorithmicif\ #1\ \algorithmicthen}
\algnewcommand{\EndIIf}{\unskip\ \algorithmicend\ \algorithmicif}

% Define "upon" keyword in algpseudocode.
\algdef{SE}% flags used internally to indicate we're defining a new block statement
[UPON]% new block type, not to be confused with loops or if-statements
{Upon}
{EndUpon}
[1]% There is one argument.
{Upon {#1}} % How begin looks.
{\textbf{end upon}} % How end looks.
\algtext*{EndUpon} % Remove end, forcefully.
% The proper way to remove them based on package flags.
% \makeatletter
% \ifthenelse{\equal{\ALG@noend}{t}}%
%   %{}
%   {\algtext*{EndUpon}}
%   {}%
% \makeatother

% Define "when" keyword in algpseudocode.
\algdef{SE}% flags used internally to indicate we're defining a new block statement
[WHEN]% new block type, not to be confused with loops or if-statements
{When}
{EndWhen}
[1]% There is one argument.
{When {#1}} % How begin looks.
{\textbf{end when}} % How end looks.
\algtext*{EndWhen} % Remove end, forcefully.
%\algtext*{EndIf} % This was here before for some reason.
% The proper way to remove them based on package flags.
% \makeatletter
% \ifthenelse{\equal{\ALG@noend}{t}}%
%   %{}
%   {\algtext*{EndWhen}}
%   {}%
% \makeatother

%----- Box Environment -----------------------------------------
% v 2019.1.DT small skips
%---
 \RequirePackage{varwidth}
 \RequirePackage{color}
 \RequirePackage[most]{tcolorbox}%with most option


%----- Protocol Boxes
 \newtcolorbox{titlebox}[5]{enhanced,center,colframe=black,colback=white,boxrule={#3},arc={#2},auto outer arc,%
 breakable,pad at break*=5pt,vfill before first,before={%\par\smallskip\noindent
 },after={\par\smallskip},top=12pt,left=4pt,%
 enlarge top by=2pt,%enlarge bottom by=7pt,%
 fontupper=\small,
 title={\rule[-.3\baselineskip]{0pt}{\baselineskip}\normalsize\sffamily\bfseries #1}, varwidth boxed title*=-30pt, 
 attach boxed title to top left={yshift=-10pt,xshift=10pt}, coltitle=black,
 boxed title style={colback=white,boxrule={#5},arc={#4},auto outer arc}
 }

 \newenvironment{systembox}[1]
 {\vspace{\baselineskip}\begin{titlebox}{Functionality \normalfont #1}{2.5pt}{1pt}{3.5pt}{1pt}}
 {\end{titlebox}}

 \newenvironment{protocolbox}[1]
 {\begin{titlebox}{Protocol \normalfont #1}{0.5pt}{0.5pt}{1pt}{0.75pt}}
 {\end{titlebox}}


 \newenvironment{adaptedprotocolbox}[1]
 {\begin{titlebox}{Adapted protocol \normalfont #1}{0.5pt}{0.5pt}{1pt}{0.75pt}}
 {\end{titlebox}}
 
 
  \newenvironment{simulatorbox}[1]
 {\begin{titlebox}{Simulator \normalfont #1}{0.5pt}{0.5pt}{2pt}{0.75pt}}
 {\end{titlebox}}
 
  \newenvironment{processbox}[1]
 {\begin{titlebox}{Process \normalfont #1}{0.5pt}{0.5pt}{1pt}{0.75pt}}
 {\end{titlebox}}

 \newenvironment{algobox}[1]
 {\begin{titlebox}{Algorithm \normalfont #1}{0.5pt}{0.5pt}{1pt}{0.75pt}}
 {\end{titlebox}}
 
 \newenvironment{funcbox}[1]
 {\begin{titlebox}{Function \normalfont #1}{0.5pt}{0.5pt}{1pt}{0.75pt}}
 {\end{titlebox}}

 \newenvironment{dianabox}[1]
 {\begin{titlebox}{\normalfont #1}{0.5pt}{0.5pt}{1pt}{0.75pt}}
 {\end{titlebox}}
